Improved Approximation Algorithms for (Budgeted) Node-weighted Steiner Problems

Moss and Rabani[12] study constrained node-weighted Steiner tree problems with two independent weight values associated with each node, namely, cost and prize (or penalty). They give an O(log n)-approximation algorithm for the prize-collecting node-weighted Steiner tree problem (PCST). They use the algorithm for PCST to obtain a bicriteria (2, O(log n))-approximation algorithm for the Budgeted node-weighted Steiner tree problem. Their solution may cost up to twice the budget, but collects a factor Omega(1/log n) of the optimal prize. We improve these results from at least two aspects. Our first main result is a primal-dual O(log h)-approximation algorithm for a more general problem, prize-collecting node-weighted Steiner forest, where we have (h) demands each requesting the connectivity of a pair of vertices. Our algorithm can be seen as a greedy algorithm which reduces the number of demands by choosing a structure with minimum cost-to-reduction ratio. This natural style of argument (also used by Klein and Ravi[10] and Guha et al.[8]) leads to a much simpler algorithm than that of Moss and Rabani[12] for PCST. Our second main contribution is for the Budgeted node-weighted Steiner tree problem, which is also an improvement to [12] and [8]. In the unrooted case, we improve upon an O(log^2(n))-approximation of [8], and present an O(log n)-approximation algorithm without any budget violation. For the rooted case, where a specified vertex has to appear in the solution tree, we improve the bicriteria result of [12] to a bicriteria approximation ratio of (1+eps, O(log n)/(eps^2)) for any positive (possibly subconstant) (eps). That is, for any permissible budget violation (1+eps), we present an algorithm achieving a tradeoff in the guarantee for prize. Indeed, we show that this is almost tight for the natural linear-programming relaxation used by us as well as in [12].

==> defs.tex <==
In the \emph{\caps{Node-weighted Prize-Collecting Steiner Tree}} (PCST) framework, we are given a graph $G=(V,E)$ with $n$ vertices, a non-negative prize function $\pi: V\to \mathds{R}$, a non-negative node-weight function $w: V\to \mathds{R}$, and possibly a root vertex $r\in V$. For a set $S\subseteq V$, let $\pi(S)$ and $w(S)$ respectively denote the total prize and total weight of vertices in $S$. For a subgraph $H\subseteq G$ we may misuse the definitions by using $\pi(H)$ and $w(H)$ instead of $\pi(V(H))$ and $w(V(H))$.
%Also, define the prize to cost density of $T\subseteq G$ as $\rho(T):=\pi(T)/c(T)$.

In a Steiner tree connectivity problem, we need to find a tree $T$ connecting a subset of vertices (and possibly the root) while optimizing a certain cost function. We define four different cost functions as described in \cite{johnson00}:

\begin{itemize}
\item In the \emph{Net Worth} Maximization Problem (NW) we need to
    \begin{center}
    maximize $NW(T)=\pi(T)-w(T)$.
    \end{center}


\item In the \emph{Prize-Collecting} Minimization Problem (PC) we need to
    \begin{center}
    minimize $PC(T)=\sum_{v\notin T} \pi(v)+w(T)$.
    \end{center}


\item In the \emph{Quota Prize-Collecting Problem} (QPC) given a prize quota $Q$, we need to
    \begin{center}
    minimize $w(T)$ subject to $\pi(T)\geq Q$.
    \end{center}


\item In the \emph{Budgeted Prize-Collecting Problem} (BPC) given a weight budget $B$, we need to
    \begin{center}
    maximize $\pi(T)$ subject to $w(T)\leq B$.
    \end{center}

\end{itemize}

All four problems have a \emph{rooted} variant in which $r$ must be contained in $T$. We may also define a \emph{directed}
variant in which $G$ is directed and $T$ must be a directed tree rooted at $r$ (i.e., there is a unique directed path in $T$ from $r$ to every vertex in $T$). In what follows we consider undirected graphs unless it is specifically mentioned otherwise.

Moss and Rabani~\cite{MossRabani} were the first to consider prize-collecting Steiner connectivity problems with node weights. They design an $O(\log n)$-approximation algorithm for the PC and Quota problems. They also give a bicriteria approximation algorithm for the budgeted variant. Recall that in the budgeted problem the goal is to maximize the prize while respecting a budget limit. The later finds a tree with the total prize at least $\frac{1}{O(\log n)}$ fraction of the prize of optimal solution, however, the weight of the tree may violate the budget by a factor of two. It is proven difficult to get rid of the violation factor. One obstacle arises from the fact that most of the known results rely on the primal-dual framework of Goemans and Williamson~\cite{GW92} which leads to an inapproximability in the budgeted problem: At the heart of the algorithm of Moss and Rabani, they roughly find an integral primal solution which is within $O(\log n)$ approximation of a \emph{fractional} dual solution. Interestingly, using a simple example we show the integrality gap of the LP formulation with hard constraints is very large. Thus it is not surprising that currently there is no approximation algorithm for the rooted budgeted problem which does not violate the budget. \vlnote{Are we going to assume the following? For the unrooted version Guha et al.~\cite{Guha99} give an $O(\log^2 n)$-approximation algorithm without violation}.

The main results of the paper are an $O(\log n)$-approximation algorithm for the unrooted budgeted problem and a bicriteria approximation algorithm with approximation ratio $\left(O(\frac{\log n}{\epsilon}),(1+\epsilon)\right)$ for every $\epsilon\in(0,1]$ for the rooted version.
An $(\alpha,\beta)$-bicriteria approximation algorithm for the budgeted problem finds a tree with total prize at least $\frac{1}{\alpha}$ fraction of that of optimal solution and total weight at most $\beta$ factor of the budget.
To get over the integrality gap of the LP formulation, 
we prove several structural properties of near-optimum solutions. 
By restricting the solution to one with these properties, 
we use the bicriteria approximation algorithm of Moss and Rabani~\cite{MossRabani} 
as a black-box for finding a near-optimum solution. 
Finally we use a generalization of the trimming method of \cite{Guha99} 
to avoid violating the budget. 
In Section~\ref{sec:mossrabani} we give a much simpler algorithm for the PC problem 
and we briefly discuss the method of Moss and Rabani. 
Next, in Section~\ref{sec:budgeted} we describe our algorithms for the budgeted problem.

